LLM-augmented Preference Learning from Natural Language

Finding preferences expressed in natural language is an important but challenging task. State-of-the-art(SotA) methods leverage transformer-based models such as BERT, RoBERTa, etc. and graph neural architectures such as graph attention networks. Since Large Language Models (LLMs) are equipped to deal with larger context lengths and have much larger model sizes than the transformer-based model, we investigate their ability to classify comparative text directly. This work aims to serve as a first step towards using LLMs for the CPC task. We design and conduct a set of experiments that format the classification task into an input prompt for the LLM and a methodology to get a fixed-format response that can be automatically evaluated. Comparing performances with existing methods, we see that pre-trained LLMs are able to outperform the previous SotA models with no fine-tuning involved. Our results show that the LLMs can consistently outperform the SotA when the target text is large -- i.e. composed of multiple sentences --, and are still comparable to the SotA performance in shorter text. We also find that few-shot learning yields better performance than zero-shot learning.

==> generation.tex <==
In addition to the classification task, we use the LLM generate synthetic data to be used in the training of the smaller models.
We use the same fine-tuned LLaMa-2 70B model for this task.
Randomly selected options and few-shot examples from the original dataset are used to construct a prompt that is then passed to the LLM.
The options include the number of sentences to generate, an adjective describing the person to imitate, the role of the person to imitate, the aspect to focus on in the comment, and the sentiment of the previous comment.
We randomly choose the few-shot examples from the rows that have the same label as the comment to generate.

In this experiment, each data point generated mimics a comment on a college confidential forum. The options randomly selected for each prompt are as follows:

\begin{itemize}
    \item {\bf Number of Sentences}: 1, 2, 3, 5, 8
    \item {\bf Adjective}: happy, disgruntled, ambivalent, stressed, friendly, angry, disappointed, excited, proud, curious
    \item {\bf Role}: parent, alumni, prospective student, current student, teacher, hiring manager, faculty, admissions officer, international student
    \item {\bf Aspect}: location, faculty, career options, competitiveness, admission rates, social life, fraternities, tuition, academics, research, size, financial aid
    \item {\bf Previous Comment}: someone who agrees with you, someone who disagrees with you, someone who just got into one of the colleges, someone who just got into both of the colleges, someone who is not sure of where to apply to, a comment that discusses statistics, the start of a discussion
    \item {\bf Label}
    \begin{itemize}
        \item {\bf No Preference}: writes only objective and irrelevant comments about \{alternative\_a\} and \{alternative\_b\}
        \item {\bf Preference}: prefers \{alternative\_a\} over \{alternative\_b\} but doesn't want hurt the feelings of those that disagree with you
        \item {\bf Equal Preference}: thinks that \{alternative\_a\} and \{alternative\_b\} are equal but doesn't want to make it obvious
    \end{itemize}
\end{itemize}
These options can generate 151,200 unique prompts. 

\noindent In our experiment, we set the following LLM parameters:
\begin{itemize}
    \item {\bf temperature} (0.7): encourage more diverse responses
    \item {\bf top\_p} (0.1): ensure adherence to the guidelines
    \item {\bf repetition penalty} (1.18): encourage the LLM to talk about various aspects and prevent tunnel vision when generating comments
\end{itemize}

The prompt consists of three sections: system message, few-shot examples, and comment prompt.
We use the system message to convey a persona and the preference regarding the two choices it should have to the LLM.
The user message first introduces the examples as comments previously generated by the LLM, then asks the LLM to generate a comment while keeping the persona and preference in mind.
An example is shown below:

{\td format this better}

System Prompt
\begin{quote}
You are an expert at generating sample comments for college confidential forums.
Please pretend that you are a(n) \{adjective\} \{role\} who \{label\}.
Please write exactly \{number of sentences\} sentences.
Please talk about \{aspect\} as relevant to the colleges.
Please start your comment by talking about the colleges.
\end{quote}
User Prompt
\begin{quote}
Here are some excellent examples of comments that you have generated before for other colleges and personalities:

\triplebackticks example 1\\
\{example 1 comment\}\\
\triplebackticks

\triplebackticks example 2\\
\{example 2 comment\}\\
\triplebackticks

\triplebackticks example 3\\
\{example 3 comment\}\\
\triplebackticks

Please generate a \{number of sentences\} sentence comment that responds to \{previous comment\} and follows the original instructions.
\end{quote}
The LLM often starts comments with an introduction of itself such as ``As a disappointed alumnae of both UT Austin and Brown University...'' or ``As a stressed parent...'' when no guidelines on the start of the comment are given. 
To reduce the likelihood of this behavior, the line ``Please start your comment by talking about the colleges'' is added. 
This line is better at reducing this type of behavior than simply asking it {\it not} to start the comment with an introduction.

\noindent We try two ways to convey the persona to the LLM:
\begin{itemize}
    \item first telling the LLM that it is an expert at generating sample data, then asking it to pretend to assume the given persona
    \item directly telling the LLM that it is the given persona
\end{itemize}
\noindent Both perform similarly when no examples are provided, but with examples, the latter is more likely to reference those examples or use content from them in its generated data.

Telling the LLM that it simply believes that option A is better than option B results in a very radical comment.
It often writes its preference directly within the comment, making the task of extracting its preference trivial and thus nullifying its use as a training point.
Adding statements such as "but doesn't want hurt the feelings of those that disagree with you" and "but doesn't want to make it obvious" to the end of the assigned preference results in a more realistic comment from which it is much harder to extract the preference.


